A Theoretical Framework for R-parity Violation

We propose a theoretical framework for R-parity violation. It is realized by a class of Calabi--Yau compactification of Heterotic string theory. Trilinear R-parity violation in superpotential is either absent or negligibly small without an unbroken symmetry, due to a selection rule based on charge counting of a spontaneously broken U(1) symmetry. Although such a selection rule cannot be applied in general to non-renormalizable operators in the low-energy effective superpotential, it is valid for terms trilinear in low-energy degrees of freedom, and hence can be used as a solution to the dimension-4 proton decay problem in the minimal supersymmetric standard model. Bilinear R-parity violation is generated, but there are good reasons why they are small enough to satisfy its upper bounds from neutrino mass and washout of baryon/lepton asymmetry. All R-parity violating dimension-5 operators can be generated. In this theoretical framework, nucleons can decay through squark-exchange diagrams combining dimension-5 and bilinear R-parity violating operators. B-L breaking neutron decay is predicted.

==> M-m32_2.tex <==
%WinTpicVersion3.08
\unitlength 0.1in
\begin{picture}( 38.7000, 36.0000)(  5.9500,-37.1500)
% STR 2 0 3 0
% 3 800 700 800 800 5 0
% 2
\put(8.0000,-8.0000){\makebox(0,0){2}}%
% STR 2 0 3 0
% 3 800 900 800 1000 5 0
% 1
\put(8.0000,-10.0000){\makebox(0,0){1}}%
% STR 2 0 3 0
% 3 800 1100 800 1200 5 0
% 0
\put(8.0000,-12.0000){\makebox(0,0){0}}%
% STR 2 0 3 0
% 3 800 1300 800 1400 5 0
% -1
\put(8.0000,-14.0000){\makebox(0,0){-1}}%
% STR 2 0 3 0
% 3 800 3100 800 3200 5 0
% -10
\put(8.0000,-32.0000){\makebox(0,0){-10}}%
% VECTOR 2 0 3 0
% 2 1000 3600 1000 400
% 
\special{pn 8}%
\special{pa 1000 3600}%
\special{pa 1000 400}%
\special{fp}%
\special{sh 1}%
\special{pa 1000 400}%
\special{pa 980 468}%
\special{pa 1000 454}%
\special{pa 1020 468}%
\special{pa 1000 400}%
\special{fp}%
% STR 2 0 3 0
% 3 1400 3700 1400 3800 5 0
% 1
\put(14.0000,-38.0000){\makebox(0,0){1}}%
% STR 2 0 3 0
% 3 3400 3700 3400 3800 5 0
% 11
\put(34.0000,-38.0000){\makebox(0,0){11}}%
% STR 2 0 3 0
% 3 4000 3700 4000 3800 5 0
% 14
\put(40.0000,-38.0000){\makebox(0,0){14}}%
% VECTOR 2 0 3 0
% 2 1000 3600 4400 3600
% 
\special{pn 8}%
\special{pa 1000 3600}%
\special{pa 4400 3600}%
\special{fp}%
\special{sh 1}%
\special{pa 4400 3600}%
\special{pa 4334 3580}%
\special{pa 4348 3600}%
\special{pa 4334 3620}%
\special{pa 4400 3600}%
\special{fp}%
% LINE 2 0 3 0
% 2 4000 600 4000 1400
% 
\special{pn 8}%
\special{pa 4000 600}%
\special{pa 4000 1400}%
\special{fp}%
% LINE 2 0 3 0
% 2 3400 600 3400 3600
% 
\special{pn 8}%
\special{pa 3400 600}%
\special{pa 3400 3600}%
\special{fp}%
% LINE 2 0 3 0
% 2 1400 1200 3800 3600
% 
\special{pn 8}%
\special{pa 1400 1200}%
\special{pa 3800 3600}%
\special{fp}%
% LINE 2 2 3 0
% 2 1000 1200 1400 1200
% 
\special{pn 8}%
\special{pa 1000 1200}%
\special{pa 1400 1200}%
\special{dt 0.045}%
% LINE 2 2 3 0
% 2 1400 1200 1400 3600
% 
\special{pn 8}%
\special{pa 1400 1200}%
\special{pa 1400 3600}%
\special{dt 0.045}%
% LINE 2 2 3 0
% 2 1000 1400 4000 1400
% 
\special{pn 8}%
\special{pa 1000 1400}%
\special{pa 4000 1400}%
\special{dt 0.045}%
% LINE 2 2 3 0
% 2 4000 1400 4000 3600
% 
\special{pn 8}%
\special{pa 4000 1400}%
\special{pa 4000 3600}%
\special{dt 0.045}%
% LINE 2 2 3 0
% 2 1000 3200 3400 3200
% 
\special{pn 8}%
\special{pa 1000 3200}%
\special{pa 3400 3200}%
\special{dt 0.045}%
% VECTOR 2 0 3 0
% 2 3600 3400 3800 3400
% 
\special{pn 8}%
\special{pa 3600 3400}%
\special{pa 3800 3400}%
\special{fp}%
\special{sh 1}%
\special{pa 3800 3400}%
\special{pa 3734 3380}%
\special{pa 3748 3400}%
\special{pa 3734 3420}%
\special{pa 3800 3400}%
\special{fp}%
% STR 2 0 3 0
% 3 4200 3300 4200 3400 5 0
% $p \to KG$
\put(42.0000,-34.0000){\makebox(0,0){$p \to KG$}}%
% STR 2 0 3 0
% 3 3200 300 3200 400 5 0
% $p \to K \mu$
\put(32.0000,-4.0000){\makebox(0,0){$p \to K \mu$}}%
% STR 2 0 3 0
% 3 4200 300 4200 400 5 0
% $\tilde{\tau} \to q u^{c}$
\put(42.0000,-4.0000){\makebox(0,0){$\tilde{\tau} \to q u^{c}$}}%
% VECTOR 2 0 3 0
% 2 3400 800 3600 800
% 
\special{pn 8}%
\special{pa 3400 800}%
\special{pa 3600 800}%
\special{fp}%
\special{sh 1}%
\special{pa 3600 800}%
\special{pa 3534 780}%
\special{pa 3548 800}%
\special{pa 3534 820}%
\special{pa 3600 800}%
\special{fp}%
% VECTOR 2 0 3 0
% 2 4000 800 3800 800
% 
\special{pn 8}%
\special{pa 4000 800}%
\special{pa 3800 800}%
\special{fp}%
\special{sh 1}%
\special{pa 3800 800}%
\special{pa 3868 820}%
\special{pa 3854 800}%
\special{pa 3868 780}%
\special{pa 3800 800}%
\special{fp}%
% LINE 2 2 3 0
% 2 1000 800 2600 800
% 
\special{pn 8}%
\special{pa 1000 800}%
\special{pa 2600 800}%
\special{dt 0.045}%
% LINE 2 2 3 0
% 2 1000 1000 2400 1000
% 
\special{pn 8}%
\special{pa 1000 1000}%
\special{pa 2400 1000}%
\special{dt 0.045}%
% LINE 2 0 3 0
% 2 2400 800 2200 1000
% 
\special{pn 8}%
\special{pa 2400 800}%
\special{pa 2200 1000}%
\special{fp}%
% LINE 2 0 3 0
% 2 2600 800 2400 1000
% 
\special{pn 8}%
\special{pa 2600 800}%
\special{pa 2400 1000}%
\special{fp}%
% STR 2 0 3 0
% 3 1000 100 1000 200 5 0
% $m_{3/2}$
\put(10.0000,-2.0000){\makebox(0,0){$m_{3/2}$}}%
% STR 2 0 3 0
% 3 4600 3500 4600 3600 5 0
% $M$
\put(46.0000,-36.0000){\makebox(0,0){$M$}}%
% VECTOR 2 0 3 0
% 2 2300 900 2450 900
% 
\special{pn 8}%
\special{pa 2300 900}%
\special{pa 2450 900}%
\special{fp}%
\special{sh 1}%
\special{pa 2450 900}%
\special{pa 2384 880}%
\special{pa 2398 900}%
\special{pa 2384 920}%
\special{pa 2450 900}%
\special{fp}%
% VECTOR 2 0 3 0
% 2 2500 900 2650 900
% 
\special{pn 8}%
\special{pa 2500 900}%
\special{pa 2650 900}%
\special{fp}%
\special{sh 1}%
\special{pa 2650 900}%
\special{pa 2584 880}%
\special{pa 2598 900}%
\special{pa 2584 920}%
\special{pa 2650 900}%
\special{fp}%
% STR 2 0 3 0
% 3 2400 1100 2400 1200 5 0
% 511keV/diffuse $\gamma$
\put(24.0000,-12.0000){\makebox(0,0){511keV/diffuse $\gamma$}}%
\end{picture}%


==> fig_lsp_1b.tex <==
\begin{fmfgraph*}(50,30)
\fmfleft{i1}
\fmfright{o3}
\fmfrightn{o}{2}
\fmf{plain,t=3,la=$\hat{\tilde{\chi}}{}^0$,la.s=left}{i1,v1}
\fmf{wiggly,t=0}{i1,v1}
\fmf{wiggly,left=1,la=$W^+$,la.s=left}{v1,v2}
\fmf{phantom}{v1,v2}
\fmf{fermion,t=3,la=$\hat{\nu}$,la.s=left}{v2,o3}
\fmfshift{(-0.1w,0.05h)}{o1}
\fmffreeze
\fmf{fermion,right=0.66,la=$\tilde{H}_d^-$,la.s=right}{v1,v3}
\fmf{fermion,right=0.22,t=0.01}{v3,v2}
\fmf{wiggly,t=1.4}{v3,o1}
\fmfv{d.shape=circle,d.size=8,d.filled=shaded}{v2}
\fmfv{l=$\gamma$,l.a=0}{o1}
\end{fmfgraph*}

==> fig_lsp_1c.tex <==
\begin{fmfgraph*}(50,30)
\fmfleft{i1}
\fmfright{o3}
\fmfrightn{o}{2}
\fmf{plain,t=3,la=$\hat{\tilde{\chi}}{}^0$,la.s=left}{i1,v1}
\fmf{wiggly,t=0}{i1,v1}
\fmf{scalar,right=1,la=$H_d^-$,la.s=right}{v2,v1}
\fmf{phantom}{v1,v2}
\fmf{fermion,t=3,la=$\hat{\nu}$,la.s=left}{v2,o3}
\fmfshift{(-0.1w,0.05h)}{o1}
\fmffreeze
\fmf{fermion,left=0.66,la=$e^c$,la.s=left}{v3,v1}
\fmf{fermion,left=0.22,t=0.01}{v2,v3}
\fmf{wiggly,t=1.4}{v3,o1}
\fmfv{d.shape=circle,d.size=8,d.filled=shaded}{v1}
\fmfv{l=$\gamma$,l.a=0}{o1}
\end{fmfgraph*}

==> fig_lsp_2b.tex <==
\begin{fmfgraph*}(50,30)
\fmfleft{i1}
\fmfrightn{o}{3}
\fmf{plain,t=3,la=$\hat{\tilde{\chi}}{}^0$,la.s=left}{i1,v1}
\fmf{wiggly,t=0}{i1,v1}
\fmf{fermion}{v1,o3}
\fmf{phantom}{o1,v1}
\fmffreeze
\fmf{scalar,la=$H^0/H^\pm$,la.s=left}{v2,v1}
\fmf{fermion}{v2,o1}
\fmf{fermion,t=0.01}{v2,o2}
\fmfv{d.shape=circle,d.size=8,d.filled=shaded}{v1}
\fmfv{l=$f^c$,l.a=0}{o1}
\fmfv{l=$f$,l.a=0}{o2}
\fmfv{l=$\nu/e^\mp$,l.a=0}{o3}
\end{fmfgraph*}

==> figure3-1a.tex <==
\begin{fmfgraph*}(65,30)
\fmfleft{i1}
\fmfrightn{o}{2}
\fmf{phantom,t=2}{i1,v3}
\fmf{phantom}{o1,v3}
\fmf{phantom}{o2,v3}
\fmffreeze
\fmfshift{(0,0.05h)}{o1}
\fmfshift{(0,-0.05h)}{o2}
\fmffreeze
\fmf{fermion}{i1,v1}
\fmf{wiggly,t=0}{i1,v1}
\fmf{fermion,label=$\widetilde{H}_d^0$,label.side=right}{v1,v2}
\fmf{fermion,label=$\widetilde{H}_d^-$,label.side=right}{v2,v3}
\fmf{fermion}{v3,v4}
\fmf{fermion,label=$\widetilde{H}_d^0$,label.side=right}{v4,v5}
\fmf{fermion}{v5,o2}
\fmffreeze
\fmf{wiggly,label=$W^+$,label.side=left,left=0.8}{v2,v4}
\fmf{wiggly}{o1,v3}
\fmfv{d.shape=circle,d.size=8,d.filled=shaded,l={\scriptsize $Z_{\chi\tilde{H}_d^0}$},l.a=90}{v1}
\fmfv{d.shape=circle,d.size=8,d.filled=shaded,l={\scriptsize $Z_{\nu\tilde{H}_d^0}$},l.a=120}{v5}
\fmfv{l=$\chi$}{i1}
\fmfv{l=$\nu$}{o2}
\fmfv{l=$\gamma$}{o1}
\end{fmfgraph*}

==> figure3-1b.tex <==
\begin{fmfgraph*}(50,30)
\fmfleft{i1}
\fmfrightn{o}{3}
\fmf{phantom,t=2}{i1,v2}
\fmf{phantom}{o1,v2}
\fmf{phantom}{o3,v2}
\fmffreeze
\fmf{fermion}{i1,v1}
\fmf{wiggly,t=0}{i1,v1}
\fmf{fermion,label=$\widetilde{H}_d^0$,label.side=right}{v1,v2}
\fmf{fermion}{v2,v3}
\fmf{fermion}{v3,o3}
\fmf{wiggly,label=$Z$,label.side=right,t=5}{v2,v4}
\fmf{fermion,t=0.1}{o2,v4}
\fmf{fermion,t=4.9}{v4,o1}
\fmfv{d.shape=circle,d.size=8,d.filled=shaded,l={\scriptsize $Z_{\nu\tilde{H}_d^0}$},l.a=120}{v3}
\fmfv{d.shape=circle,d.size=8,d.filled=shaded,l={\scriptsize $Z_{\chi\tilde{H}_d^0}$},l.a=90}{v1}
\fmfv{l=$\chi$}{i1}
\fmfv{l=$\nu$}{o3}
\fmfv{l=$f$}{o1}
\fmfv{l=$\bar{f}$}{o2}
\end{fmfgraph*}

==> figure_hhh5_4.tex <==
\begin{fmfgraph*}(80,32)
\fmfleftn{i}{2}
\fmfrightn{o}{2}
\fmfright{n3}
\fmfbottomn{n}{2}
\fmf{fermion}{i1,v1}
\fmf{fermion,t=2}{i2,v1}
\fmf{fermion,t=2}{o2,v2}
\fmf{phantom,t=0.55}{v1,v2}
\fmf{phantom}{o1,v2}
\fmffreeze
\fmf{fermion,label=$\overline{N}_*$,label.side=left}{v3,v1}
\fmf{fermion,label=$\overline{N}^c_*$,label.side=right}{v3,v6}
\fmf{fermion,label=$\Phi_*$,label.side=left}{v7,v6}
\fmf{fermion,label=$\Phi_*$,label.side=right}{v7,v8}
\fmf{fermion,label=$\overline{N}^c_*$,label.side=left}{v9,v8}
\fmf{fermion,label=$\overline{N}_*$,label.side=right}{v9,v2}
\fmf{fermion,label=$\bar{\bf 5}_*$,label.side=right,label.d=2}{v4,v2}
\fmf{fermion,label=$\bar{\bf 5}^c_*$,label.side=left,label.d=2}{v4,v5}
\fmf{fermion}{o1,v5}
\fmffreeze
\fmfshift{(0.38w,0.45h)}{n1}
\fmfshift{(-0.38w,0.45h)}{n2}
\fmfshift{(0,-0.22h)}{n3}
\fmf{fermion}{n1,v6}
\fmf{fermion}{n2,v8}
\fmf{fermion}{n3,v5}
\fmfv{d.shape=cross,d.size=8,d.angle=25}{v4}
\fmfv{d.shape=cross,d.size=8,d.angle=0}{v3}
\fmfv{d.shape=cross,d.size=8,d.angle=0}{v7}
\fmfv{d.shape=cross,d.size=8,d.angle=0}{v9}
\fmfv{l=$\bar{\bf 5}_0$,l.a=180}{i1}
\fmfv{l=$H_0$,l.a=180}{i2}
\fmfv{l=$\bar{H}_0$,l.a=0}{o1}
\fmfv{l=$H_0$,l.a=0}{o2}
\fmfv{l=$\langle\overline{N}\rangle$,l.a=-110,l.d=3}{n1}
\fmfv{l=$\langle\overline{N}\rangle$,l.a=-70,l.d=3}{n2}
\fmfv{l=$\langle\overline{N}\rangle$,l.a=20,l.d=3}{n3}
\fmfv{l={\scriptsize $y^\nu_{(1)}$},l.a=180}{v1}
\fmfv{l={\scriptsize $y^\nu_{(1)}$},l.a=115,l.d=2.5}{v2}
\fmfv{l={\scriptsize $M_{\bar{\bf 5}}$},l.a=-150,l.d=3}{v4}
\fmfv{l={\scriptsize $y^\nu_{(2)}$},l.a=-150,l.d=1}{v5}
\fmfv{l={\scriptsize $M_N$},l.a=90}{v3}
\fmfv{l={\scriptsize $y''^\nu_{(2)}$},l.a=90,l.d=3}{v6}
\fmfv{l={\scriptsize $M_\Phi$},l.a=90}{v7}
\fmfv{l={\scriptsize $y''^\nu_{(2)}$},l.a=90,l.d=3}{v8}
\fmfv{l={\scriptsize $M_N$},l.a=90}{v9}
\end{fmfgraph*}

==> figure_neut-tri-decay1.tex <==
\begin{fmfgraph*}(40,25)
\fmfleft{i1}
\fmfrightn{o}{3}
\fmf{fermion,t=7}{i1,v4}
\fmf{wiggly,t=0}{i1,v1}
\fmf{fermion,t=7,label=$\tilde{B}$,label.side=left}{v4,v1}
\fmf{scalar,t=4,label=$\tilde{\nu}_L$,label.side=right,label.d=3}{v1,v2}
\fmf{fermion,t=4}{o1,v2}
\fmf{fermion}{o2,v2}
\fmf{fermion,t=1.5}{o3,v1}
\fmfv{d.shape=circle,d.size=8,d.filled=shaded,l={\scriptsize $Z_{\chi \tilde{B}}$},l.a=-90}{v4}
\fmfv{l=$\chi$,l.a=90}{i1}
\fmfv{l=$d_L$,l.a=0}{o1}
\fmfv{l=$d^c$,l.a=0}{o2}
\fmfv{l=$\nu_L$,l.a=0}{o3}
\fmfv{l={\scriptsize $\lambda'_{ijk}$},l.a=-90,l.d=2}{v2}
\end{fmfgraph*}

==> figure_neutdecay1.tex <==
\begin{fmfgraph*}(40,25)
\fmfleft{i1}
\fmfrightn{o}{3}
\fmf{plain,t=4}{i1,v1}
\fmf{boson}{i1,v1}
\fmf{scalar,t=4,label=$\tilde{e^c}$,label.side=left}{v2,v1}
\fmf{fermion,t=4}{v2,o1}
\fmf{fermion}{v2,o2}
\fmf{fermion,t=1.5}{v1,o3}
\fmfv{l=$\tilde{\chi}_0$,l.a=90}{i1}
\fmfv{l=$d_L$,l.a=0}{o1}
\fmfv{l=$u^c$,l.a=0}{o2}
\fmfv{l=$e^c$,l.a=0}{o3}
\fmfv{l=$\langle h_d\rangle$,l.a=-110}{v2}
\end{fmfgraph*}

==> figure_neutdecay2.tex <==
\begin{fmfgraph*}(40,25)
\fmfleft{i1}
\fmfrightn{o}{3}
\fmf{plain,t=4}{i1,v1}
\fmf{boson}{i1,v1}
\fmf{scalar,t=4,label=$\tilde{d}_L$,label.side=left}{v2,v1}
\fmf{fermion,t=4}{v2,o1}
\fmf{fermion}{v2,o2}
\fmf{fermion,t=1.5}{v1,o3}
\fmfv{l=$\tilde{\chi}_0$,l.a=90}{i1}
\fmfv{l=$u^c$,l.a=0}{o1}
\fmfv{l=$e^c$,l.a=0}{o2}
\fmfv{l=$d_L$,l.a=0}{o3}
\fmfv{l=$\langle h_d\rangle$,l.a=-110}{v2}
\end{fmfgraph*}

==> figure_neutdecay3.tex <==
\begin{fmfgraph*}(40,25)
\fmfleft{i1}
\fmfrightn{o}{3}
\fmf{plain,t=4}{i1,v1}
\fmf{boson}{i1,v1}
\fmf{scalar,t=4,label=$\tilde{u}^c$,label.side=left}{v2,v1}
\fmf{fermion,t=4}{v2,o1}
\fmf{fermion}{v2,o2}
\fmf{fermion,t=1.5}{v1,o3}
\fmfv{l=$\tilde{\chi}_0$,l.a=90}{i1}
\fmfv{l=$e^c$,l.a=0}{o1}
\fmfv{l=$d_L$,l.a=0}{o2}
\fmfv{l=$u^c$,l.a=0}{o3}
\fmfv{l=$\langle h_d\rangle$,l.a=-110}{v2}
\end{fmfgraph*}

==> figure_neutdecay4.tex <==
\begin{fmfgraph*}(40,25)
\fmfleft{i1}
\fmfrightn{o}{3}
\fmf{plain,t=4}{i1,v1}
\fmf{boson}{i1,v1}
\fmf{scalar,t=4,label=$\tilde{q}_L$,label.side=left}{v2,v1}
\fmf{fermion,t=4}{v2,o1}
\fmf{fermion}{v2,o2}
\fmf{fermion,t=1.5}{v1,o3}
\fmfv{l=$\tilde{\chi}_0$,l.a=90}{i1}
\fmfv{l=$q_L$,l.a=0}{o1}
\fmfv{l=$q_L$,l.a=0}{o2}
\fmfv{l=$q_L$,l.a=0}{o3}
\fmfv{l=$\langle h_d\rangle$,l.a=-112}{v2}
\end{fmfgraph*}

==> figure_pdecay1.tex <==
\begin{fmfgraph*}(50,35)
\fmfleftn{i}{3}
\fmfrightn{o}{3}
\fmffreeze
\fmfshift{(0,0.3h)}{i2,o2}
\fmfshift{(0,-0.1h)}{i3,o3}
\fmf{fermion,right=0.1}{i3,o3}
\fmf{fermion}{i2,v1}
\fmf{fermion}{o2,v1}
\fmf{scalar,label=$\tilde{s}_L$,t=0.4,left=0.5}{v2,v1}
\fmf{scalar,label=$h_d{}^0$,t=0.4,right=0.5}{v2,v1}
\fmf{fermion}{v2,i1}
\fmf{fermion}{v2,o1}
\fmfv{l=$u$,l.a=90}{i3,o3}
\fmfv{l=$d_L$,l.a=-90}{i2}
\fmfv{l=$\bar{u}_L$,l.a=-90}{o2}
\fmfv{l=$\bar{u}^c$,l.a=90}{i1}
\fmfv{l=$e^c$,l.a=90}{o1}
\end{fmfgraph*}

==> figure_pdecay2.tex <==
\begin{fmfgraph*}(50,35)
\fmfleftn{i}{3}
\fmfrightn{o}{3}
\fmffreeze
\fmfshift{(0,0.3h)}{i2,o2}
\fmfshift{(0,-0.1h)}{i3,o3}
\fmf{fermion,right=0.1}{i3,o3}
\fmf{fermion}{i2,v1}
\fmf{fermion}{o2,v1}
\fmf{scalar,label=$\tilde{s}_L$,t=1.3}{v2,v1}
\fmf{fermion}{v2,i1}
\fmf{fermion}{v2,o1}
\fmfv{l=$u$,l.a=90}{i3,o3}
\fmfv{l=$d_L$,l.a=-90}{i2}
\fmfv{l=$\bar{u}_L$,l.a=-90}{o2}
\fmfv{l=$\bar{u}^c$,l.a=90}{i1}
\fmfv{l=$e^c$,l.a=90}{o1}
\fmfv{l=$\langle h_d \rangle$,l.a=90}{v1}
\fmfv{l=$\langle h_d \rangle$,l.a=-90}{v2}
\end{fmfgraph*}

==> figure_pdecay3.tex <==
\begin{fmfgraph*}(65,45)
\fmfleftn{i}{3}
\fmfrightn{o}{3}
\fmfleftn{bl}{3}
\fmfrightn{br}{5}
\fmftopn{bt}{2}
\fmfbottomn{bb}{2}
\fmfshift{(0.1w,0.275h)}{i2}
\fmfshift{(-0.1w,0.275h)}{o2}
\fmfshift{(0.1w,0.1h)}{i1}
\fmfshift{(-0.1w,0.1h)}{o1}
\fmfshift{(0.1w,-0.1h)}{i3}
\fmfshift{(-0.1w,-0.1h)}{o3}
\fmfshift{(0.05w,0)}{bb1,bt1}
\fmfshift{(-0.05w,0.4h)}{br2}
\fmfshift{(0,0.15h)}{br3}
\fmfshift{(0,0.075h)}{br4}
\fmfshift{(-0.05w,0)}{bt2}
\fmf{fermion,r=0.1}{i3,o3}
\fmf{fermion,t=1.4}{i1,v1}
\fmf{fermion,t=1.4}{i2,v2}
\fmf{phantom,t=1}{v1,v2}
\fmf{scalar,la=$\tilde{d}_L$,la.s=left}{v4,v2}
\fmf{scalar,la=$\tilde{\nu}_L$,la.s=right}{v3,v1}
\fmf{plain,t=0.01}{v3,v4}
\fmf{wiggly,t=0}{v3,v4}
\fmf{fermion,t=1.4}{o1,v3}
\fmf{fermion,t=1.4}{o2,v4}
\fmf{plain}{bb1,bl1,bl3,bt1}
\fmf{plain}{bt2,br5,br3,br2}
\fmffreeze
\fmf{fermion,la=$\tilde{h}_c$,la.s=right}{v5,v1}
\fmf{fermion,la=$\tilde{\bar{h}}_c$,la.s=left}{v5,v2}
\fmfv{d.sh=cross,d.si=8,d.a=0}{v5}
\fmfv{l=$u_L$,l.a=-90}{i2}
\fmfv{l=$d_L$,l.a=90}{i1}
\fmfv{l=$u_L$,l.a=-90}{o2}
\fmfv{l=$e_L$,l.a=0}{o1}
\fmfv{l=$u/d$,l.a=60}{i3}
\fmfv{l=$u/d$,l.a=120}{o3}
\fmfv{l=$p/n$,l.a=180}{bl2}
\fmfv{l=$\pi^0/\pi^-$,l.a=0}{br4}
\end{fmfgraph*}

==> figure_pdecay4.tex <==
\begin{fmfgraph*}(65,45)
\fmfleftn{i}{3}
\fmfrightn{o}{3}
\fmfleftn{bl}{3}
\fmfrightn{br}{5}
\fmftopn{bt}{2}
\fmfbottomn{bb}{2}
\fmfshift{(0.1w,0.275h)}{i2}
\fmfshift{(-0.1w,0.275h)}{o2}
\fmfshift{(0.1w,0.1h)}{i1}
\fmfshift{(-0.1w,0.1h)}{o1}
\fmfshift{(0.1w,-0.1h)}{i3}
\fmfshift{(-0.1w,-0.1h)}{o3}
\fmfshift{(0.05w,0)}{bb1,bt1}
\fmfshift{(-0.05w,0.4h)}{br2}
\fmfshift{(0,0.15h)}{br3}
\fmfshift{(0,0.075h)}{br4}
\fmfshift{(-0.05w,0)}{bt2}
\fmf{fermion,r=0.1}{i3,o3}
\fmf{fermion}{i2,v1,i1}
\fmf{wiggly,la=$X_\mu$,la.s=right,t=1.5}{v1,v2}
\fmf{fermion}{o2,v2,o1}
\fmf{plain}{bb1,bl1,bl3,bt1}
\fmf{plain}{bt2,br5,br3,br2}
\fmfv{l=$d_L$,l.a=-105}{i2}
\fmfv{l=$u^c$,l.a=105}{i1}
\fmfv{l=$u_L$,l.a=-75}{o2}
\fmfv{l=$e^c$,l.a=0}{o1}
\fmfv{l=$u/d$,l.a=60}{i3}
\fmfv{l=$u/d$,l.a=120}{o3}
\fmfv{l=$p/n$,l.a=180}{bl2}
\fmfv{l=$\pi^0/\pi^-$,l.a=0}{br4}
\end{fmfgraph*}

==> figure_pdecay5.tex <==
\begin{fmfgraph*}(65,45)
\fmfleftn{i}{3}
\fmfrightn{o}{3}
\fmfleftn{bl}{3}
\fmfrightn{br}{5}
\fmftopn{bt}{2}
\fmfbottomn{bb}{2}
\fmfshift{(0.1w,0.275h)}{i2}
\fmfshift{(-0.1w,0.275h)}{o2}
\fmfshift{(0.1w,0.1h)}{i1}
\fmfshift{(-0.1w,0.1h)}{o1}
\fmfshift{(0.1w,-0.1h)}{i3}
\fmfshift{(-0.1w,-0.1h)}{o3}
\fmfshift{(0.05w,0)}{bb1,bt1}
\fmfshift{(-0.05w,0.4h)}{br2}
\fmfshift{(0,0.15h)}{br3}
\fmfshift{(0,0.075h)}{br4}
\fmfshift{(-0.05w,0)}{bt2}
\fmf{fermion,r=0.1}{i3,o3}
\fmf{fermion}{i2,v1}
\fmf{fermion}{i1,v1}
\fmf{scalar,la=$\tilde{u}_L$,la.s=right,t=1.5}{v2,v1}
\fmf{fermion}{v2,o1}
\fmf{fermion}{v2,o2}
\fmf{plain}{bb1,bl1,bl3,bt1}
\fmf{plain}{bt2,br5,br3,br2}
\fmfv{l=$d_L$,l.a=-105}{i2}
\fmfv{l=$d_L$,l.a=105}{i1}
\fmfv{l=$d^c$,l.a=-75}{o2}
\fmfv{l=$e_L$,l.a=0}{o1}
\fmfv{l=$\vev{h_d}$,l.a=-75}{v1}
\fmfv{l=$u$,l.a=60}{i3}
\fmfv{l=$u$,l.a=120}{o3}
\fmfv{l=$n$,l.a=180}{bl2}
\fmfv{l=$\pi^+$,l.a=0}{br4}
\end{fmfgraph*}

==> figure_pdecay6.tex <==
\begin{fmfgraph*}(65,45)
\fmfleftn{i}{3}
\fmfrightn{o}{3}
\fmfleftn{bl}{3}
\fmfrightn{br}{5}
\fmftopn{bt}{2}
\fmfbottomn{bb}{2}
\fmfshift{(0.1w,0.275h)}{i2}
\fmfshift{(-0.1w,0.275h)}{o2}
\fmfshift{(0.1w,0.1h)}{i1}
\fmfshift{(-0.1w,0.1h)}{o1}
\fmfshift{(0.1w,-0.1h)}{i3}
\fmfshift{(-0.1w,-0.1h)}{o3}
\fmfshift{(0.05w,0)}{bb1,bt1}
\fmfshift{(-0.05w,0.4h)}{br2}
\fmfshift{(0,0.15h)}{br3}
\fmfshift{(0,0.075h)}{br4}
\fmfshift{(-0.05w,0)}{bt2}
\fmf{fermion,r=0.1}{i3,o3}
\fmf{fermion}{i2,v1}
\fmf{fermion}{i1,v1}
\fmf{scalar,la=$\tilde{d}_L$,la.s=right,t=1.5}{v2,v1}
\fmf{dbl_plain}{v2,o1}
\fmf{fermion}{o2,v2}
\fmf{plain}{bb1,bl1,bl3,bt1}
\fmf{plain}{bt2,br5,br3,br2}
\fmfv{l=$u_L$,l.a=-105}{i2}
\fmfv{l=$d_L$,l.a=105}{i1}
\fmfv{l=$d_L$,l.a=-75}{o2}
\fmfv{l=$\psi_{3/2}$,l.a=0}{o1}
\fmfv{l=$\vev{h_d}$,l.a=-75}{v1}
\fmfv{l=$u/d$,l.a=60}{i3}
\fmfv{l=$u/d$,l.a=120}{o3}
\fmfv{l=$p/n$,l.a=180}{bl2}
\fmfv{l=$\pi^+/\pi^0$,l.a=0}{br4}
\end{fmfgraph*}

==> figure_pndecay1.tex <==
\begin{fmfgraph*}(65,45)
\fmfleftn{i}{3}
\fmfrightn{o}{3}
\fmfleftn{bl}{3}
\fmfrightn{br}{5}
\fmftopn{bt}{2}
\fmfbottomn{bb}{2}
\fmfshift{(0.1w,0.275h)}{i2}
\fmfshift{(-0.1w,0.275h)}{o2}
\fmfshift{(0.1w,0.1h)}{i1}
\fmfshift{(-0.1w,0.1h)}{o1}
\fmfshift{(0.1w,-0.1h)}{i3}
\fmfshift{(-0.1w,-0.1h)}{o3}
\fmfshift{(0.05w,0)}{bb1,bt1}
\fmfshift{(-0.05w,0.4h)}{br2}
\fmfshift{(0,0.15h)}{br3}
\fmfshift{(0,0.075h)}{br4}
\fmfshift{(-0.05w,0)}{bt2}
\fmf{fermion,r=0.1,la=$u$,la.s=left}{i3,o3}
\fmf{fermion}{i2,v1}
\fmf{fermion}{i1,v1}
\fmf{scalar,la=$\tilde{d}_L$,la.s=right,t=1.5}{v2,v1}
\fmf{fermion,la=$\nu_L$,la.s=right}{v2,o1}
\fmf{fermion}{v2,o2}
\fmf{plain}{bb1,bl1,bl3,bt1}
\fmf{plain}{bt2,br5,br3,br2}
\fmfv{l=$u_L$,l.a=-105}{i2}
\fmfv{l=$d_L$,l.a=105}{i1}
\fmfv{l=$d^c$,l.a=-75}{o2}
\fmfv{l=$\nu$,l.a=0}{o1}
\fmfv{l={\scriptsize $\frac{\vev{H_d^0}}{M_3}$},l.a=-75}{v1}
\fmfv{l={\scriptsize $\lambda'_{ijk}$},l.a=-105}{v2}
\fmfv{l=$p$,l.a=180}{bl2}
\fmfv{l=$M^+$,l.a=0}{br4}
\end{fmfgraph*}

==> figure_pndecay2.tex <==
\begin{fmfgraph*}(65,45)
\fmfleftn{i}{3}
\fmfrightn{o}{3}
\fmfleftn{bl}{3}
\fmfrightn{br}{5}
\fmftopn{bt}{2}
\fmfbottomn{bb}{2}
\fmfshift{(0.1w,0.275h)}{i2}
\fmfshift{(-0.1w,0.275h)}{o2}
\fmfshift{(0.1w,0.1h)}{i1}
\fmfshift{(-0.1w,0.1h)}{o1}
\fmfshift{(0.1w,-0.1h)}{i3}
\fmfshift{(-0.1w,-0.1h)}{o3}
\fmfshift{(0.05w,0)}{bb1,bt1}
\fmfshift{(-0.05w,0.4h)}{br2}
\fmfshift{(0,0.15h)}{br3}
\fmfshift{(0,0.075h)}{br4}
\fmfshift{(-0.05w,0)}{bt2}
\fmf{fermion,r=0.1,la=$u$,la.s=left}{i3,o3}
\fmf{fermion}{i2,v1}
\fmf{fermion}{v1,i1}
\fmf{scalar,la=$\tilde{d}_L$,la.s=right,t=1.5}{v2,v1}
\fmf{fermion,la=$\nu_L$,la.s=right}{v2,o1}
\fmf{fermion}{v2,o2}
\fmf{plain}{bb1,bl1,bl3,bt1}
\fmf{plain}{bt2,br5,br3,br2}
\fmfv{l=$u_L$,l.a=-105}{i2}
\fmfv{l=$d^c$,l.a=105}{i1}
\fmfv{l=$d^c$,l.a=-75}{o2}
\fmfv{l=$\nu$,l.a=0}{o1}
\fmfv{l={\scriptsize $\frac{\partial}{M_7}$},l.a=-75}{v1}
\fmfv{l={\scriptsize $\lambda'_{ijk}$},l.a=-105}{v2}
\fmfv{l=$p$,l.a=180}{bl2}
\fmfv{l=$M^+$,l.a=0}{br4}
\end{fmfgraph*}

==> figure_stau-decay1.tex <==
\begin{fmfgraph*}(40,20)
\fmfleft{i1}
\fmfrightn{o}{2}
\fmf{scalar,t=3}{i1,v1}
\fmf{phantom}{o1,v1}
\fmf{fermion}{o2,v1}
\fmffreeze
\fmf{fermion}{o1,v2}
\fmf{fermion,la=$\widetilde{H}_d^0$,la.s=left,la.d=3}{v2,v1}
\fmfv{d.shape=circle,d.size=8,d.filled=shaded}{v2}
\fmfv{l=$\tilde{\tau}^c$,l.a=90}{i1}
\fmfv{l=$\nu_{Lk}$,l.a=0}{o1}
\fmfv{l=$\tau_L$,l.a=0}{o2}
\fmfv{l={\scriptsize $Z_{\nu\widetilde{H}_{\!d}}$},l.a=-110}{v2}
\end{fmfgraph*}

==> figure_stau-decay2.tex <==
\begin{fmfgraph*}(40,20)
\fmfleft{i1}
\fmfrightn{o}{2}
\fmf{scalar,t=3}{i1,v1}
\fmf{fermion}{o1,v1}
\fmf{fermion}{o2,v1}
\fmfv{l=$\tilde{\tau}^c$,l.a=90}{i1}
\fmfv{l=$\nu_{Lk}$,l.a=0}{o1}
\fmfv{l=$\tau_{L}$,l.a=0}{o2}
\fmfv{l={\scriptsize $\lambda_{33k}$},l.a=-110}{v1}
\end{fmfgraph*}

==> figure_stau-decay3.tex <==
\begin{fmfgraph*}(40,20)
\fmfleft{i1}
\fmfrightn{o}{2}
\fmf{scalar,t=3}{i1,v1}
\fmf{fermion}{o1,v1}
\fmf{fermion}{o2,v1}
\fmfv{l=$\tilde{\tau}^c$,l.a=90}{i1}
\fmfv{l=$d_L$,l.a=0}{o1}
\fmfv{l=$u^c$,l.a=0}{o2}
\fmfv{l={\scriptsize $\frac{\langle H_d^0\rangle}{M_4}$},l.a=-110}{v1}
\end{fmfgraph*}

==> figure_staudecay1.tex <==
\begin{fmfgraph*}(40,20)
\fmfleft{i1}
\fmfrightn{o}{2}
\fmf{scalar,t=2}{i1,v1}
\fmf{fermion}{o1,v1}
\fmf{fermion}{o2,v1}
\fmfv{l=$\tilde{\tau}$,l.a=90}{i1}
\fmfv{l=$d_L$,l.a=0}{o1}
\fmfv{l=$u^c$,l.a=0}{o2}
\fmfv{l=$\langle h_d\rangle$,l.a=-110}{v1}
\end{fmfgraph*}

==> figure_staudecay2.tex <==
\begin{fmfgraph*}(40,20)
\fmfleft{i1}
\fmfrightn{o}{3}
\fmf{scalar,t=3}{i1,v1}
\fmf{fermion}{o1,v1}
\fmf{fermion}{o2,v1}
\fmf{scalar}{o3,v1}
\fmfv{l=$\tilde{\tau}$,l.a=90}{i1}
\fmfv{l=$d_L$,l.a=0}{o1}
\fmfv{l=$u^c$,l.a=0}{o2}
\fmfv{l=$h$,l.a=0}{o3}
\end{fmfgraph*}
